Sampling Matters: The Effect of ECG Frequency on Deep Learning-Based Atrial Fibrillation Detection

Deep learning models for atrial fibrillation (AF) detection are increasingly trained on heterogeneous electrocardiogram (ECG) datasets with varying sampling frequencies, yet the specific consequences of these discrepancies on model performance, calibration, and robustness remain insufficiently characterized. To address this, we conducted a systematic benchmark using 12-lead, 10-second recordings from the PTB-XL dataset, resampled to target frequencies of 62, 100, 250, and 500 Hz, to evaluate a standard 1-D Convolutional Neural Network (CNN) and a hybrid CNN-Long Short-Term Memory (LSTM) architecture under a rigorous patient-safe cross-validation framework. Our analysis reveals that sampling frequency significantly impacts detection metrics in an architecture-dependent manner; the hybrid CNN-LSTM model demonstrated optimal performance and consistent calibration at intermediate frequencies (100-250 Hz), whereas the 1-D CNN baseline exhibited marked degradation in accuracy and sensitivity at 500 Hz, suggesting increased susceptibility to high-frequency noise. We conclude that ECG sampling frequency is a critical, underappreciated factor in arrhythmia detection, and future foundation models must explicitly control for temporal resolution to ensure clinical reliability and reproducibility.

==> Tables/combined_val_test_single_header_dataset_model.tex <==
% Requires: \usepackage{booktabs}
\begin{table*}[!t]
\centering
\caption{Validation (5-fold cross-validation) and final imbalanced test performance across ECG sampling frequencies.
Validation metrics are reported as mean $\pm$ standard deviation across folds. ECE $\downarrow$ indicates lower is better.}
\label{tab:val_test_sampling_combined}
\footnotesize
\setlength{\tabcolsep}{3.9pt}
\renewcommand{\arraystretch}{1.10}

\resizebox{\textwidth}{!}{
\begin{tabular}{lllcccccccc}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{Frequency} &
\textbf{Accuracy} & \textbf{F1} & \textbf{Precision} &
\textbf{Sensitivity} & \textbf{Specificity} & \textbf{MCC} &
\textbf{AUROC} & \textbf{ECE $\downarrow$} \\
\midrule
\multirow{8}{*}{Validation}  & CNN--LSTM & 62 Hz & $0.9844 \pm 0.0074$ & $0.9844 \pm 0.0075$ & $0.9873 \pm 0.0078$ & $0.9816 \pm 0.0156$ & $0.9873 \pm 0.0076$ & $0.9691 \pm 0.0149$ & $0.9952 \pm 0.0040$ & $0.021 \pm 0.002$ \\
 & CNN--LSTM & 100 Hz & $0.9821 \pm 0.0087$ & $0.9820 \pm 0.0089$ & $0.9855 \pm 0.0103$ & $0.9788 \pm 0.0165$ & $0.9854 \pm 0.0102$ & $0.9644 \pm 0.0173$ & $0.9937 \pm 0.0043$ & $0.028 \pm 0.012$ \\
 & CNN--LSTM & 250 Hz & \textbf{$0.9878 \pm 0.0047$} & \textbf{$0.9877 \pm 0.0048$} & \textbf{$0.9922 \pm 0.0066$} & \textbf{$0.9835 \pm 0.0135$} & \textbf{$0.9922 \pm 0.0065$} & \textbf{$0.9758 \pm 0.0095$} & $0.9941 \pm 0.0060$ & \textbf{$0.020 \pm 0.006$} \\
 & CNN--LSTM & 500 Hz & $0.9849 \pm 0.0090$ & $0.9847 \pm 0.0091$ & $0.9911 \pm 0.0038$ & $0.9786 \pm 0.0175$ & $0.9912 \pm 0.0037$ & $0.9701 \pm 0.0180$ & \textbf{$0.9963 \pm 0.0034$} & $0.026 \pm 0.013$ \\
 \cmidrule(lr){2-11}
 & CNN1D & 62 Hz & $0.9859 \pm 0.0052$ & $0.9858 \pm 0.0053$ & \textbf{$0.9893 \pm 0.0032$} & $0.9825 \pm 0.0100$ & \textbf{$0.9893 \pm 0.0033$} & $0.9719 \pm 0.0106$ & $0.9956 \pm 0.0041$ & $0.020 \pm 0.005$ \\
 & CNN1D & 100 Hz & \textbf{$0.9874 \pm 0.0079$} & \textbf{$0.9873 \pm 0.0080$} & \textbf{$0.9893 \pm 0.0058$} & \textbf{$0.9854 \pm 0.0150$} & \textbf{$0.9893 \pm 0.0057$} & \textbf{$0.9748 \pm 0.0159$} & \textbf{$0.9966 \pm 0.0037$} & \textbf{$0.018 \pm 0.006$} \\
 & CNN1D & 250 Hz & $0.9781 \pm 0.0049$ & $0.9781 \pm 0.0051$ & $0.9740 \pm 0.0073$ & $0.9825 \pm 0.0125$ & $0.9737 \pm 0.0074$ & $0.9564 \pm 0.0102$ & $0.9960 \pm 0.0032$ & $0.027 \pm 0.005$ \\
 & CNN1D & 500 Hz & $0.9519 \pm 0.0132$ & $0.9509 \pm 0.0135$ & $0.9679 \pm 0.0117$ & $0.9349 \pm 0.0241$ & $0.9688 \pm 0.0115$ & $0.9046 \pm 0.0264$ & $0.9857 \pm 0.0048$ & $0.038 \pm 0.010$ \\
 \midrule
\multirow{8}{*}{Test}  & CNN--LSTM & 62 Hz & 0.9884 & 0.9581 & 0.9295 & 0.9581 & 0.9884 & 0.9520 & 0.9983 & 0.015 \\
 & CNN--LSTM & 100 Hz & 0.9905 & 0.9657 & 0.9417 & 0.9657 & 0.9905 & 0.9606 & 0.9984 & 0.011 \\
 & CNN--LSTM & 250 Hz & 0.9905 & 0.9657 & 0.9417 & 0.9657 & 0.9905 & 0.9606 & 0.9983 & 0.011 \\
 & CNN--LSTM & 500 Hz & 0.9887 & 0.9587 & 0.9429 & 0.9587 & 0.9908 & 0.9523 & 0.9977 & 0.011 \\
  \cmidrule(lr){2-11}
 & CNN1D & 62 Hz & 0.9844 & 0.9445 & 0.9061 & 0.9445 & 0.9841 & 0.9366 & 0.9975 & 0.017 \\
 & CNN1D & 100 Hz & 0.9860 & 0.9495 & 0.9191 & 0.9495 & 0.9866 & 0.9420 & 0.9972 & 0.015 \\
 & CNN1D & 250 Hz & 0.9811 & 0.9328 & 0.8921 & 0.9328 & 0.9817 & 0.9231 & 0.9969 & 0.027 \\
 & CNN1D & 500 Hz & 0.9707 & 0.8963 & 0.8539 & 0.8963 & 0.9750 & 0.8808 & 0.9899 & 0.038 \\
\bottomrule
\end{tabular}
}
\vspace{-10pt}
\end{table*}


==> Tables/combined_val_test_tables.tex <==
% Requires: \usepackage{booktabs,siunitx}
\begin{table*}[!t]
\centering
\caption{Performance comparison across ECG sampling frequencies on both
validation (5-fold cross-validation) and imbalanced test set.
All validation metrics are reported as mean $\pm$ standard deviation across folds.
ECE $\downarrow$ indicates lower is better.}
\label{tab:val_test_sampling}
\footnotesize
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.12}

\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Frequency} &
\textbf{Accuracy} & \textbf{F1} & \textbf{Precision} &
\textbf{Sensitivity} & \textbf{Specificity} &
\textbf{MCC} & \textbf{AUROC} & \textbf{ECE $\downarrow$} \\
\midrule

\multicolumn{9}{l}{\textbf{Validation Set (5-Fold Cross-Validation)}} \\
\midrule
\multicolumn{9}{l}{\textbf{CNN--LSTM}} \\
\midrule
62 Hz  & $0.9844 \pm 0.0074$ & $0.9844 \pm 0.0075$ & $0.9873 \pm 0.0078$ & $0.9816 \pm 0.0156$ & $0.9873 \pm 0.0076$ & $0.9691 \pm 0.0149$ & $0.9952 \pm 0.0040$ & $0.021 \pm 0.002$ \\
100 Hz & $0.9821 \pm 0.0087$ & $0.9820 \pm 0.0089$ & $0.9855 \pm 0.0103$ & $0.9788 \pm 0.0165$ & $0.9854 \pm 0.0102$ & $0.9644 \pm 0.0173$ & $0.9937 \pm 0.0043$ & $0.028 \pm 0.012$ \\
250 Hz & \textbf{$0.9878 \pm 0.0047$} & \textbf{$0.9877 \pm 0.0048$} & \textbf{$0.9922 \pm 0.0066$} & \textbf{$0.9835 \pm 0.0135$} & \textbf{$0.9922 \pm 0.0065$} & \textbf{$0.9758 \pm 0.0095$} & $0.9941 \pm 0.0060$ & \textbf{$0.020 \pm 0.006$} \\
500 Hz & $0.9849 \pm 0.0090$ & $0.9847 \pm 0.0091$ & $0.9911 \pm 0.0038$ & $0.9786 \pm 0.0175$ & $0.9912 \pm 0.0037$ & $0.9701 \pm 0.0180$ & \textbf{$0.9963 \pm 0.0034$} & $0.026 \pm 0.013$ \\

\addlinespace[0.4em]
\multicolumn{9}{l}{\textbf{Test Set (Imbalanced, AF prevalence = 0.1344)}} \\
\midrule
\multicolumn{9}{l}{\textbf{CNN--LSTM}} \\
\midrule
62 Hz  & 0.9884 & 0.9581 & 0.9295 & 0.9581 & 0.9884 & 0.9520 & 0.9983 & 0.0151 \\
100 Hz & 0.9905 & 0.9657 & 0.9417 & 0.9657 & 0.9905 & 0.9606 & 0.9984 & 0.0111 \\
250 Hz & 0.9905 & 0.9657 & 0.9417 & 0.9657 & 0.9905 & 0.9606 & 0.9983 & 0.0108 \\
500 Hz & 0.9887 & 0.9587 & 0.9429 & 0.9587 & 0.9908 & 0.9523 & 0.9977 & 0.0108 \\

\bottomrule
\end{tabular}
}
\end{table*}

==> Tables/results.tex <==
% Requires: \usepackage{booktabs}

\begin{table*}[!t]
\centering
\caption{Validation performance across ECG sampling frequencies using
5-fold cross-validation.
All metrics are reported as mean $\pm$ standard deviation across folds.
Sensitivity was evaluated at a fixed decision threshold of 0.5,
AUROC was computed from validation probabilities, and Expected
Calibration Error (ECE) was computed from validation softmax
probabilities $\mathrm{softmax}(\mathbf{z})[:,1]$ (lower is better).}
\label{tab:val_sampling}
\footnotesize
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.15}

\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Frequency} &
\textbf{Accuracy} & \textbf{F1} & \textbf{Precision} &
\textbf{Specificity} & \textbf{MCC} &
\textbf{Sensitivity} & \textbf{AUROC} & \textbf{ECE $\downarrow$} \\
\midrule

\multicolumn{9}{l}{\textbf{CNN--LSTM}} \\
\midrule
62 Hz  &
$0.9844 \pm 0.0074$ &
$0.9844 \pm 0.0075$ &
$0.9873 \pm 0.0078$ &
$0.9873 \pm 0.0076$ &
$0.9691 \pm 0.0149$ &
$0.9816 \pm 0.0156$ &
$0.9952 \pm 0.0040$ &
$0.021 \pm 0.002$ \\

100 Hz &
$0.9821 \pm 0.0087$ &
$0.9820 \pm 0.0089$ &
$0.9855 \pm 0.0103$ &
$0.9854 \pm 0.0102$ &
$0.9644 \pm 0.0173$ &
$0.9788 \pm 0.0165$ &
$0.9937 \pm 0.0043$ &
$0.028 \pm 0.012$ \\

250 Hz &
\textbf{$0.9878 \pm 0.0047$} &
\textbf{$0.9877 \pm 0.0048$} &
\textbf{$0.9922 \pm 0.0066$} &
\textbf{$0.9922 \pm 0.0065$} &
\textbf{$0.9758 \pm 0.0095$} &
\textbf{$0.9835 \pm 0.0135$} &
$0.9941 \pm 0.0060$ &
\textbf{$0.020 \pm 0.006$} \\

500 Hz &
$0.9849 \pm 0.0090$ &
$0.9847 \pm 0.0091$ &
$0.9911 \pm 0.0038$ &
$0.9912 \pm 0.0037$ &
$0.9701 \pm 0.0180$ &
$0.9786 \pm 0.0175$ &
\textbf{$0.9963 \pm 0.0034$} &
$0.026 \pm 0.013$ \\

\addlinespace[0.35em]
\midrule
\multicolumn{9}{l}{\textbf{CNN1D}} \\
\midrule

62 Hz &
$0.9859 \pm 0.0052$ &
$0.9858 \pm 0.0053$ &
\textbf{$0.9893 \pm 0.0032$} &
\textbf{$0.9893 \pm 0.0033$} &
$0.9719 \pm 0.0106$ &
$0.9825 \pm 0.0100$ &
$0.9956 \pm 0.0041$ &
$0.020 \pm 0.005$ \\

100 Hz &
\textbf{$0.9874 \pm 0.0079$} &
\textbf{$0.9873 \pm 0.0080$} &
\textbf{$0.9893 \pm 0.0058$} &
\textbf{$0.9893 \pm 0.0057$} &
\textbf{$0.9748 \pm 0.0159$} &
\textbf{$0.9854 \pm 0.0150$} &
\textbf{$0.9966 \pm 0.0037$} &
\textbf{$0.018 \pm 0.006$} \\

250 Hz &
$0.9781 \pm 0.0049$ &
$0.9781 \pm 0.0051$ &
$0.9740 \pm 0.0073$ &
$0.9737 \pm 0.0074$ &
$0.9564 \pm 0.0102$ &
$0.9825 \pm 0.0125$ &
$0.9960 \pm 0.0032$ &
$0.027 \pm 0.005$ \\

500 Hz &
$0.9519 \pm 0.0132$ &
$0.9509 \pm 0.0135$ &
$0.9679 \pm 0.0117$ &
$0.9688 \pm 0.0115$ &
$0.9046 \pm 0.0264$ &
$0.9349 \pm 0.0241$ &
$0.9857 \pm 0.0048$ &
$0.038 \pm 0.010$ \\

\bottomrule
\end{tabular}
}
\end{table*}


==> Tables/test_unbalances_table.tex <==
\begin{table*}[!t]
\centering
\caption{Final test performance obtained using an ensemble of the
best-performing model from each cross-validation fold.
All results are reported on the naturally imbalanced test set
(AF prevalence = 0.1344), reflecting real clinical conditions.
ECE is computed using positive-class probability calibration.
$\overline{P(\mathrm{AF})}$ denotes the mean predicted AF probability.}

\label{tab:test_sampling}
\footnotesize
\setlength{\tabcolsep}{3.9pt}
\renewcommand{\arraystretch}{1.08}

\begin{tabular}{
l
S S S S S S
S S
S
}
\toprule
\textbf{Frequency} &
\textbf{Acc.} & \textbf{F1} & \textbf{Prec.} &
\textbf{Sens.} & \textbf{Spec.} & \textbf{MCC} &
\textbf{AUROC} & \textbf{ECE} &
\boldmath$\overline{P(\mathrm{AF})}$ \\
\midrule

\multicolumn{10}{c}{\textbf{CNN--LSTM}} \\
\midrule

62\,Hz  & 0.9884 & 0.9581 & 0.9295 & 0.9581 & 0.9884 & 0.9520 & 0.9983 & 0.0151 & 0.1494 \\
100\,Hz & 0.9905 & 0.9657 & 0.9417 & 0.9657 & 0.9905 & 0.9606 & 0.9984 & 0.0111 & 0.1454 \\
250\,Hz & 0.9905 & 0.9657 & 0.9417 & 0.9657 & 0.9905 & 0.9606 & 0.9983 & 0.0108 & 0.1452 \\
500\,Hz & 0.9887 & 0.9587 & 0.9429 & 0.9587 & 0.9908 & 0.9523 & 0.9977 & 0.0108 & 0.1448 \\

\addlinespace[0.4em]
\midrule
\multicolumn{10}{c}{\textbf{CNN1D}} \\
\midrule

62\,Hz  & 0.9844 & 0.9445 & 0.9061 & 0.9445 & 0.9841 & 0.9366 & 0.9975 & 0.0168 & 0.1511 \\
100\,Hz & 0.9860 & 0.9495 & 0.9191 & 0.9495 & 0.9866 & 0.9420 & 0.9972 & 0.0147 & 0.1491 \\
250\,Hz & 0.9811 & 0.9328 & 0.8921 & 0.9328 & 0.9817 & 0.9231 & 0.9969 & 0.0267 & 0.1610 \\
500\,Hz & 0.9707 & 0.8963 & 0.8539 & 0.8963 & 0.9750 & 0.8808 & 0.9899 & 0.0378 & 0.1721 \\

\bottomrule
\end{tabular}
\end{table*}


==> figures/tikz_figure.tex <==
\begin{figure*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=stealth,
    % General text box styles with expanded widths for Rows 1 & 3
    r1box/.style={draw, rectangle, rounded corners, align=center, fill=blue!5, font=\small, minimum height=1.5cm},
    r3box/.style={draw, rectangle, rounded corners, align=center, fill=blue!5, font=\small, minimum height=1.5cm},
    % Row 2 specific styles
    cnnbox/.style={draw, rectangle, rounded corners, align=center, text width=2.6cm, minimum height=1.5cm, fill=orange!10, font=\scriptsize},
    lstmbox/.style={draw, rectangle, rounded corners, align=center, text width=2.6cm, minimum height=1.5cm, fill=green!10, font=\scriptsize},
    decision/.style={draw, diamond, aspect=1.3, align=center, fill=green!5, font=\small\bfseries, inner sep=2pt},
    r2box/.style={draw, rectangle, rounded corners, align=center, fill=blue!5, font=\scriptsize, minimum height=1.5cm},
    % Bounding box and arrow styles
    rowbox/.style={draw, rectangle, rounded corners, inner sep=12pt, dashed, fill=gray!5},
    title/.style={font=\large\bfseries, align=left},
    arrow/.style={thick, ->},
    % FIX: Added braces around Latex to prevent pgfkeys comma parsing errors. Size reduced.
    thickarrow/.style={-{Latex[length=3mm, width=3mm]}, line width=1.5mm, draw=black!60}
]

% ================= INVISIBLE BOUNDARY NODES =================
% These dummy nodes force all three dashed row boxes to have the exact same width
% Adjusted Y-coordinates to reduce the gaps between the rows
\node (W1) at (-2.5, 5.2) {}; \node (E1) at (29.5, 5.2) {};
\node (W2) at (-2.5, 0) {}; \node (E2) at (29.5, 0) {};
\node (W3) at (-2.5, -4.5) {}; \node (E3) at (29.5, -4.5) {};

% ================= ROW 1: PRE-PROCESSING & DATA LOADING =================
\node[title] (title1) at (-2.2, 6.7) [anchor=north west] {Data Pre-Processing \& Fold-Specific Data Loading};

\node[r1box, text width=3.5cm] (raw) at (0, 5.2) {Raw ECG datasets\\(PTB-XL)};
\node[r1box, text width=4cm] (filter) at (6, 5.2) {Label filtering:\\AFIB vs NORMAL\\+ patient\_id};
\node[r1box, text width=6.5cm] (preproc) at (13, 5.2) {Signal preprocessing: NaN/Inf cleaning, clipping,\\Resampling (62-500Hz), z-score normalization,\\10-s segmentation};
\node[r1box, text width=4.5cm] (split) at (20, 5.2) {Patient-safe partitioning:\\Hold-out test split\\Stratified K-fold};
\node[r1box, text width=5cm] (dataload) at (26.5, 5.2) {Fold-Specific Loading:\\Read data.pt + CSV\\Select validation fold, DataLoaders};

\draw[arrow] (raw) -- (filter);
\draw[arrow] (filter) -- (preproc);
\draw[arrow] (preproc) -- (split);
\draw[arrow] (split) -- (dataload);

\begin{scope}[on background layer]
    \node[rowbox, fit=(W1) (E1) (title1) (raw) (dataload)] (R1) {};
\end{scope}

% ================= ROW 2: MODEL CHOICE & TRAINING =================
\node[title] (title2) at (-2.2, 3.0) [anchor=north west] {Model Choice \& Training};

\node[decision, text width=2cm] (choice) at (0, 0) {Model\\Choice};

% CNN1D Path (Top)
\node[cnnbox] (c1) at (3.5, 1.5) {Conv1D (C$\rightarrow$32, k=7)\\BN+ReLU. MaxPool(2)};
\node[cnnbox] (c2) at (7.0, 1.5) {Conv1D (32$\rightarrow$64, k=5)\\BN+ReLU. MaxPool(2)};
\node[cnnbox] (c3) at (10.5, 1.5) {Conv1D (64$\rightarrow$128, k=5)\\BN+ReLU. MaxPool(2)};
\node[cnnbox] (c4) at (14.0, 1.5) {Conv1D (128$\rightarrow$256, k=3)\\BN+ReLU.\\AdaptiveAvgPool1D(1)};
\node[cnnbox] (c5) at (17.5, 1.5) {Flatten.\\Dropout FC\\(256$\rightarrow$2)};

% CNN-LSTM Path (Bottom)
\node[lstmbox] (l1) at (3.5, -1.5) {8x ShortcutConvBlock1D\\(k=10) BN, Conv1D,\\ReLU+Drop, Avg/MaxPool\\Concat. $T\rightarrow T'/2$};
\node[lstmbox] (l2) at (7.0, -1.5) {Feature map\\(256 x $T'$)};
\node[lstmbox] (l3) at (10.5, -1.5) {Permute ($T'$ x 256)\\LSTM (hidden=128)};
\node[lstmbox] (l4) at (14.0, -1.5) {Temporal\\mean pooling};
\node[lstmbox] (l5) at (17.5, -1.5) {Dropout FC\\(128$\rightarrow$2)};

% Convergence Nodes
\node[r2box, text width=3cm] (train) at (21.3, 0) {Training loop (CE)\\LR sched., class weights\\Log: loss, AUROC, F1};
\node[r2box, text width=2.2cm] (stop) at (24.3, 0) {Early stop on\\Val F1};
\node[r2box, text width=2.2cm] (save) at (27.2, 0) {Save best model\\per fold};

% Row 2 Arrows
\draw[arrow] (choice.east) -- ++(0.4,0) |- (c1.west);
\draw[arrow] (choice.east) -- ++(0.4,0) |- (l1.west);
\draw[arrow] (c1) -- (c2); \draw[arrow] (c2) -- (c3); \draw[arrow] (c3) -- (c4); \draw[arrow] (c4) -- (c5);
\draw[arrow] (l1) -- (l2); \draw[arrow] (l2) -- (l3); \draw[arrow] (l3) -- (l4); \draw[arrow] (l4) -- (l5);
\draw[arrow] (c5.east) -- ++(0.4,0) |- (train.west);
\draw[arrow] (l5.east) -- ++(0.4,0) |- (train.west);
\draw[arrow] (train) -- (stop);
\draw[arrow] (stop) -- (save);

\begin{scope}[on background layer]
    \node[rowbox, fit=(W2) (E2) (title2) (choice) (c1) (l1) (save)] (R2) {};
\end{scope}

% ================= ROW 3: TEST EVALUATION =================
\node[title] (title3) at (-2.2, -3.3) [anchor=north west] {Test Evaluation};

\node[r3box, text width=4cm] (load) at (0, -4.8) {Load best.pt\\(K folds)};
\node[r3box, text width=4.5cm] (ensemble) at (8, -4.8) {Logit averaging\\ensemble};
\node[r3box, text width=7cm] (eval) at (17, -4.8) {Test evaluation (Hold-out test split)\\Balanced \& Unbalanced datasets};
\node[r3box, text width=5cm] (metrics) at (26.5, -4.8) {Metrics: Sensitivity, Specificity,\\MCC, AUROC, F1};

\draw[arrow] (load) -- (ensemble);
\draw[arrow] (ensemble) -- (eval);
\draw[arrow] (eval) -- (metrics);

\begin{scope}[on background layer]
    \node[rowbox, fit=(W3) (E3) (title3) (load) (metrics)] (R3) {};
\end{scope}

% ================= INTER-ROW THICK ARROWS =================
\draw[thickarrow] (R1.south) -- (R2.north);
\draw[thickarrow] (R2.south) -- (R3.north);

\end{tikzpicture}
}
\caption{Overview of the proposed experimental pipeline. Raw 12-lead ECG recordings are preprocessed, resampled to multiple target sampling frequencies, segmented into fixed-length windows, and split using patient-safe cross-validation. Identical deep learning models are then trained and evaluated at each frequency to analyze performance, calibration, and cross-frequency robustness.}
\label{fig:experimental_pipeline}
\end{figure*}
